Unavailable Transit Feed Specification: Making it Available with Recurrent Neural Networks

Studies on public transportation in Europe suggest that European inhabitants use buses in ca. 56% of all public transport travels. One of the critical factors affecting such a percentage and more, in general, the demand for public transport services, with an increasing reluctance to use them, is their quality. End-users can perceive quality from various perspectives, including the availability of information, i.e., the access to details about the transit and the provided services. The approach proposed in this paper, using innovative methodologies resorting on data mining and machine learning techniques, aims to make available the unavailable data about public transport. In particular, by mining GPS traces, we manage to reconstruct the complete transit graph of public transport. The approach has been successfully validated on a real dataset collected from the local bus system of the city of L'Aquila (Italy). The experimental results demonstrate that the proposed approach and implemented framework are both effective and efficient, thus being ready for deployment.

==> src/running-example.tex <==

\section{Background}\label{sec:running-ex}

In this section, we present a motivating example.

\subsection{Motivating Example}

Some of the transport agencies are still providing services to users as years ago. Technological advancements are done only in the direction of the transport agency and not to provide new services to the user. In Italy, we have multiple examples as highlighted from the rank for smart cities available at~\cite{providelink}. Here as can be noticed, multiple cities are on top for info mobility and others are on the bottom of the rank for the same. Most of the cases this is due to the user perception of the provided services, often wholly absent. L'Aquila is one example of working public transport but limited info mobility services. The transport agency still provides the timetable and other info as pdf document through their websites or other means. An example of data made available is reported in Fig.~\ref{fig:timetable}. 
In this figure, an excerpt of the available information on the website are reported. On top, a screenshot of the website of the transit agency reports the main bus stops of the selected route and the last update time. Moreover, the routes are also reported as the timeline in the centre of the screenshot. At the bottom of the screen, also the map of the covered path is represented. The timeline in the centre is linked using a pdf document, the map a jpg/png picture. Moreover, the last update highlights that those documents have to be updated for every change the agency applies.

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=\columnwidth]{figs/collage.png}
		\caption{Available information for Public Transport in L'Aquila with focus on line 3}
		\label{fig:timetable}
	\end{center}
\end{figure}

When the software involved in the management of the schedules, does not also provide a frontend for the travel planning and does not support the export in a format that can be processed by open source software, managers are stuck in a situation of vendor lock-in. 

A first solution could be arranged processing documents and convert data to GTFS standard. The General Transit Feed Specification (GTFS)\footnote{https://developers.google.com/transit/gtfs} defines a standard format for public transportation schedules and associated geographical information. GTFS enables public transit agencies to publish their transit data and developers to write applications that consume such data in an interoperable way. Multiple projects allow to convert excel spreadsheets into GTFS feed, but as expected, the input format is not universal, and the transformation process needs to be customized every time. But, this operation is time-consuming, error-prone, and it has to be repeated every time the schedule changes.
 
\begin{figure*}[h!]
	\begin{center}
		\includegraphics[width=2\columnwidth]{figs/OTP.png}
		\caption{Screenshot of OTP with imported data of line 3R}
		\label{fig:OTP}
	\end{center}
\end{figure*}
For this reason we abandoned the idea of building a communication layer from the website and data provided as in Fig.~\ref{fig:timetable} to GTFS that can be used to feed one of the open source platforms or Google directly. This is also particularly overcomplicated when multiple transit agencies are involved and the management is delegated to multiple support companies. Indeed, this process is not generic and has to be replicated for all the data sources, e.g., spreadsheets online. Moreover, the only automatic process that can be used to grab this content is HTML scraping, if the data owner does not have the resources to expose it as a machine-readable service (e.g., RESTful web service). 

To show what would be the result of the import of those data we imported some of the lines included in the excel published and converted into GTFS format. The result of this manual operation is visible in Fig.~\ref{fig:OTP}, where the same line reported in the JPG attached to the website in Fig.~\ref{fig:timetable}. Importing the GTFS provided within the OTP platform allows to plan a trip  going for instance from the source to the final destination of the reported line. The user can fill the search form with the required source and destination and the platform will return the path on the map, including the bus stops on the path. 

For all these scenarios where data are not available, in Section~\ref{sec:approach} we propose an automatic approach that using machine learning and GPS data transmitted from the buses, reconstruct the missing information, and then process them in order to produce GTFS feeds. This process will enable the usage of platforms for exposing info to the users, for instance OTP Platform. 
%Section~\ref{sec:approach} highlights the proposed approach.

%is demonstrated in section~\ref{sec:approach}, whereas the background needed to understand the section is shown in section~\ref{sec:background}.


\subsection{Recurrent Neural Networks}



==> src/threads.tex <==
\section{Limitations}\label{sec:limitations}
One of the limitation of the approach is the precision of the GPS position when GPS is not available. It can happen that in specific points the route is individuated with strange directions as in Fig.~\ref{fig:limitation1}. This can be partially solved fine-tuning the \emph{update time frequency} of the device, e.g., every 10 seconds at the moment.




\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=\columnwidth]{figs/limitation1.png}
		\caption{Limitation to be discussed}
		\label{fig:limitation1}
	\end{center}
	\vspace{-0.5cm}
\end{figure}
